Silent Subversion: Sensor Spoofing Attacks via Supply Chain Implants in Satellite Systems

Spoofing attacks are among the most destructive cyber threats to terrestrial systems, and they become even more dangerous in space, where satellites cannot be easily serviced, and operators depend on accurate telemetry to ensure mission success. When telemetry is compromised, entire spaceborne missions are placed at risk. Prior work on spoofing has largely focused on attacks from Earth, such as injecting falsified uplinks or overpowering downlinks with stronger radios. In contrast, onboard spoofing originating from within the satellite itself remains an underexplored and underanalyzed threat. This vector is particularly concerning given that modern satellites, especially small satellites, rely on modular architectures and globalized supply chains that reduce cost and accelerate development but also introduce hidden risks. This paper presents an end-to-end demonstration of an internal satellite spoofing attack delivered through a compromised vendor-supplied component implemented in NASA's NOS3 simulation environment. Our rogue Core Flight Software application passed integration and generated packets in the correct format and cadence that the COSMOS ground station accepted as legitimate. By undermining both onboard estimators and ground operator views, the attack directly threatens mission integrity and availability, as corrupted telemetry can bias navigation, conceal subsystem failures, and mislead operators into executing harmful maneuvers. These results expose component-level telemetry spoofing as an overlooked supply-chain vector distinct from jamming or external signal injection. We conclude by discussing practical countermeasures-including authenticated telemetry, component attestation, provenance tracking, and lightweight runtime monitoring-and highlight the trade-offs required to secure resource-constrained small satellites.

==> Sections/ethics.tex <==
This work was conducted in alignment with the Menlo Report principles of respect for persons, beneficence, justice, and respect for law and public interest. All experiments were performed exclusively within NASA’s \textit{Operational Simulator for Small Satellites} (NOS3), a publicly available simulation environment. No real spacecraft hardware, software, or operational networks were accessed or modified at any stage of this research.

The prototype malicious component described in this paper was implemented solely as a proof-of-concept within NOS3 to evaluate the feasibility of supply-chain style spoofing attacks. The component has not been realized outside of the simulator and cannot be deployed on live systems without significant modification. Our focus was to highlight architectural blind spots and to motivate defensive research, not to enable misuse.

We are engaged in responsible disclosure to NASA, emphasizing that the results demonstrate a class of risks rather than an immediately exploitable vulnerability in any specific mission. Simulation-only code and pseudocode abstractions are available upon request; no deployable exploits or sensitive configuration files have been released. This balance ensures reproducibility and scientific transparency while minimizing risk of dual-use harm.

Overall, the research was designed to inform and protect the satellite community by exposing overlooked attack vectors in a safe, controlled setting, while adhering to both ethical research guidelines and legal boundaries.

